Consistent Approximations for the Optimal Control of Constrained Switched Systems

Though switched dynamical systems have shown great utility in modeling a variety of physical phenomena, the construction of an optimal control of such systems has proven difficult since it demands some type of optimal mode scheduling. In this paper, we devise an algorithm for the computation of an optimal control of constrained nonlinear switched dynamical systems. The control parameter for such systems include a continuous-valued input and discrete-valued input, where the latter corresponds to the mode of the switched system that is active at a particular instance in time. Our approach, which we prove converges to local minimizers of the constrained optimal control problem, first relaxes the discrete-valued input, then performs traditional optimal control, and then projects the constructed relaxed discrete-valued input back to a pure discrete-valued input by employing an extension to the classical Chattering Lemma that we prove. We extend this algorithm by formulating a computationally implementable algorithm which works by discretizing the time interval over which the switched dynamical system is defined. Importantly, we prove that this implementable algorithm constructs a sequence of points by recursive application that converge to the local minimizers of the original constrained optimal control problem. Four simulation experiments are included to validate the theoretical developments.

==> Sections/consistent_approximation.tex <==
\subsection{Consistent Approximation}

\begin{lemma}
  \label{lemma:discrete_mu_upper_bound}
  Let $\alpha \in (0,1)$, $\beta \in (0,1)$, nd $\delta > 0$.
  Then there exists $M^*_\delta < \infty$ such that for each $N \in \N$, $\tau \in {\cal T}_N$, and $\xi \in {\cal X}_{\tau,r}$, $\theta_\tau(\xi) \leq - \delta$ implies that $\mu_\tau(\xi) \leq M^*_\delta$.
\end{lemma}
\begin{proof}
  Given $\xi' \in {\cal X}$ and $\lambda \in [0,1]$, using the Mean Value Theorem and Corollary \ref{corollary:discretized_DJ_lipschitz} we have that there exists $s \in (0,1)$ such that
  \begin{equation}
    \label{eq:dmuub_J_mvt}
    \begin{aligned}
      J_\tau \bigl( \xi + \lambda (\xi' - \xi) \bigr) - J_\tau(\xi) 
      &= \d{J_\tau}\bigl( \xi + s \lambda ( \xi' - \xi ); \lambda (\xi' - \xi) \bigr) \\
      &\leq \lambda \d{J_\tau}\bigl( \xi; \xi' - \xi \bigr) + L \lambda^2 \| \xi' - \xi \|^2_{\cal X}.
    \end{aligned}
  \end{equation}
  Letting ${\cal A}_\tau(\xi) = \left\{ (j,i) \in {\cal J} \times \{ 0, \ldots, \card{\tau} \} \mid \Psi_\tau(\xi) = \psi_{\tau,j,\tau_i}(\xi) \right\}$, then there exists a pair $(j,i) \in {\cal A}_\tau\bigl( \xi + \lambda (\xi' - \xi) \bigr)$ and $s \in (0,1)$ such that, using Corollary \ref{corollary:Dhj_lipschitz},
  \begin{equation}
    \label{eq:dmuub_psi_mvt}
    \begin{aligned}
      \Psi_\tau\bigl( \xi + \lambda (\xi' - \xi) \bigr) - \Psi_\tau(\xi) 
      &\leq \psi_{\tau,j,\tau_i}\bigl( \xi + \lambda ( \xi' - \xi ) \bigr) - \Psi_\tau(\xi) \\
      &\leq \psi_{\tau,j,\tau_i}\bigl( \xi + \lambda ( \xi' - \xi ) \bigr) - \psi_{\tau,j,\tau_k}(\xi) \\
      &= \d{\psi_{\tau,j,\tau_i}}\bigl( \xi + s \lambda ( \xi' - \xi ); \lambda ( \xi' - \xi ) \bigr) \\
      &\leq \lambda \d{\psi_{\tau,j,\tau_i}}\bigl( \xi; \xi' - \xi \bigr) + L \lambda^2 \| \xi' - \xi \|^2_{\cal X}.
    \end{aligned}
  \end{equation}

  Now let us assume that $\Psi_\tau(\xi) \leq 0$, and consider $g_\tau$ as defined in Equation \eqref{eq:discrete_theta}. Then
  \begin{equation}
    \label{eq:dmuub_theta}
    \theta_\tau(\xi) = \max \left\{ \d{J_\tau}( \xi; g_\tau(\xi) - \xi ), 
    \max_{(j,i) \in {\cal J} \times \{ 0, \ldots, \card{\tau} \}} \D{\psi_{\tau,j,\tau_i}}( \xi; g_\tau(\xi) - \xi ) 
    + \gamma \Psi_\tau(\xi) \right\} 
    \leq -\delta,
  \end{equation}
  and using Equation \eqref{eq:dmuub_J_mvt},
  \begin{equation}
    J_\tau\bigl( \xi + \beta^k ( g_\tau(\xi) - \xi ) \bigr) - J_\tau(\xi) - \alpha \beta^k \theta_\tau(\xi) 
    \leq - ( 1 - \alpha ) \delta \beta^k + 4 A^2 L \beta^{2k},
  \end{equation}
  where $A = \max\big\{ \|u\|_2 + 1 \mid u \in U \big\}$. 
  Hence, for each $k \in \N$ such that $\beta^k \leq \frac{ (1-\alpha) \delta }{ 4 A^2 L}$ we have that
  \begin{equation}
    \label{eq:dmuub_res_1}
    J_\tau\bigl( \xi + \beta^k ( g(\xi) - \xi ) \bigr) - J_\tau(\xi) \leq \alpha \beta^k \theta_\tau(\xi).
  \end{equation}
  Similarly, using Equations \eqref{eq:dmuub_psi_mvt} and \eqref{eq:dmuub_theta},
  \begin{equation}
    \Psi_\tau\bigl( \xi + \beta^k ( g(\xi) - \xi ) \bigr) - \Psi_\tau(\xi) 
    + \beta^k \bigl( \gamma \Psi_\tau(\xi) - \alpha \theta_\tau(\xi) \bigr)
    \leq - \delta \beta^k + 4 A^2 L \beta^{2k},
  \end{equation}
  hence for each $k \in \N$ such that $\beta^k \leq \min\left\{\frac{ (1-\alpha) \delta}{4 A^2 L}, \frac{1}{\gamma} \right\}$ we have that
  \begin{equation}
    \label{eq:dmuub_res_2}
    \Psi_\tau\bigl( \xi + \beta^k ( g(\xi) - \xi ) \bigr) - \alpha \beta^k \theta_\tau(\xi) 
    \leq \left( 1 - \beta^k \gamma \right) \Psi_\tau(\xi) \leq 0.
  \end{equation}

  If $\Psi_\tau(\xi) > 0$ then 
  \begin{equation}
    \max_{(j,i) \in {\cal J} \times \{ 0, \ldots, \card{\tau}\} } \D{\psi_{\tau,j,\tau_i}}( \xi; g_\tau(\xi) - \xi ) 
    \leq \theta_\tau(\xi) \leq -\delta,
  \end{equation}
  thus, from Equation \eqref{eq:dmuub_psi_mvt},
  \begin{equation}
    \Psi_\tau\big( \xi + \beta^k ( g_\tau(\xi) - \xi ) \big) - \Psi_\tau(\xi) - \alpha \beta^k \theta_\tau(\xi) 
    \leq - ( 1 - \alpha ) \delta \beta^k + 4 A^2 L \beta^{2k}.
  \end{equation}
  Hence, for each $k \in \N$ such that $\beta^k \leq \frac{ (1-\alpha) \delta}{4 A^2 L}$ we have that
  \begin{equation}
    \label{eq:dmuub_res_3}
    \Psi_\tau\bigl( \xi + \beta^k ( g_\tau(\xi) - \xi ) \bigr) - \Psi_\tau(\xi) \leq \alpha \beta^k \theta_\tau(\xi).    
  \end{equation}

  Finally, let 
  \begin{equation}
    M^*_\delta = 1 + \max \left\{ \log_{\beta} \left( \frac{ (1-\alpha) \delta}{4 A^2 L} \right), \log_{\beta} \left( \frac{1}{\gamma} \right) \right\},
  \end{equation}
  then from Equations \eqref{eq:dmuub_res_1}, \eqref{eq:dmuub_res_2}, and \eqref{eq:dmuub_res_3}, we get that $\mu_\tau(\xi) \leq M^*_\delta$ as desired.
\end{proof}

The proof of the following corollary follows directly from the estimates of $M^*_\delta$ in the proof of Lemma \ref{lemma:discrete_mu_upper_bound}.
\begin{corollary}
  \label{corollary:discrete_mu_upper_bound}
  There exists $\delta_0 > 0$ and $C > 0$ such that for each $\delta \in (0,\delta_0)$, $\theta_\tau(\xi) \leq - \delta$ implies that $\mu_\tau(\xi) \leq 1 + \log_\beta( C \delta )$.
\end{corollary}

\begin{lemma}
  \label{lemma:discrete_state_approx}
  Consider $\rho_N$ defined as in Equation \eqref{eq:rho} and $\sigma_N$ defined as in Equation \eqref{eq:sigmaN_def}.
  There exists $K > 0$ such that for each $N_0,N \in \N$, $\tau \in {\cal T}_{N_0}$, and $\xi = (u,d) \in {\cal X}_{r,\tau}$,
  \begin{equation}
    % \bigl\| x_{\sigma_N(\xi)}^{(\rho_N(\xi))}(t) - x_\tau^{(\xi)}(t) \bigr\|
    \bigl\| \phi_{\sigma_N(\xi),t}\bigl( \rho_N(\xi) \bigr) - \phi_{\tau,t}(\xi) \bigr\|
    \leq K \left( \left( \frac{1}{\sqrt{2}} \right)^N \bigl( \|\xi\|_{BV} + 1 \bigr) + \left( \frac{1}{2} \right)^{N_0} \right),
  \end{equation}
\end{lemma}
\begin{proof}
  Using the triangular inequality we have that
  \begin{multline}
    \bigl\| \phi_{\sigma_N(\xi),1}\bigl( \rho_N(\xi) \bigr) - \phi_{\tau,1}(\xi) \bigr\|_2 
    \leq \bigl\| \phi_{\sigma_N(\xi),1} \bigl( \rho_N(\xi) \bigr) - \phi_1 \bigl( \rho_N(\xi) \bigr) \bigr\|_2 +
      \bigl\| \phi_1 \bigl( \rho_N(\xi) \bigr) - \phi_1(\xi) \bigr\|_2 + \\
    + \bigl\| \phi_1 (\xi) - \phi_{\tau,1}(\xi) \bigr\|_2.
  \end{multline}
  Thus, by Theorem \ref{thm:quality_of_approximation} and Lemma \ref{lemma:convergence_discretized_traj_xi} there exists $K_1$, $K_2$, and $K_3$ such that
  \begin{equation}
    \bigl\| \phi_{\sigma_N(\xi),1}\bigl( \rho_N(\xi) \bigr) - \phi_{\tau,1}(\xi) \bigr\|_2 
    \leq K_1 \left( \frac{1}{\sqrt{2}} \right)^N \bigl( \|\xi\|_{BV} + 1 \bigr) + \frac{K_2}{2^N} + \frac{K_3}{2^{N_0}},
  \end{equation}
  hence the result follows after organizing the constants and noting that $2^{\frac{N}{2}} \leq 2^N$ for each $N \in \N$.
\end{proof}


\begin{lemma}
  \label{lemma:discrete_nu_upper_bound}
  Let $N_0 \in \N$, $\tau_0 \in {\cal T}_{N_0}$, and $\xi \in {\cal X}_{\tau,r}$. If $\theta(\xi) < 0$ then for each $\eta \in \N$ there exists a finite $N \geq N_0$ such that $\nu_{\sigma_N(\xi)}(\xi,N+\eta)$ is finite.
\end{lemma}
\begin{proof}
  Recall $\nu_\tau$, as defined in Equation \eqref{eq:discrete_nu}, is infinity only when the optimization problem it solves is not feasible. 
  To simplify our notation, let $\xi' \in {\cal X}_{\sigma_N(\xi),r}$ defined by $\xi' = \xi + \beta^{\mu_{\sigma_N(\xi)}(\xi)} \bigl( g_{\sigma_N(\xi)}(\xi) - \xi \bigr)$. 
  Then, using Lemma \ref{lemma:discrete_state_approx}, for $k \in \N$, $k \in [N,N+\eta]$, 
  \begin{equation}
    \begin{aligned}
      J_{\sigma_k(\xi')}\bigl( \rho_k(\xi') \bigr) - J_{\sigma_N(\xi)}(\xi') 
      &\leq L K \left( \left( \frac{1}{\sqrt{2}} \right)^k \left( \|\xi'\|_{BV} + 1 \right) + \left( \frac{1}{2} \right)^N \right) \\
      &\leq L K \left( \frac{1}{\sqrt{2}} \right)^N \left( \|\xi'\|_{BV} + 2 \right) \\
    \end{aligned}
  \end{equation}
  
  Also, from Lemma \ref{lemma:discretized_theta_convergence} we know that for $N$ large enough,
  \begin{equation}
    \frac{1}{2} \theta(\xi) \geq \theta_{\sigma_N(\xi)}(\xi).
  \end{equation}
  Thus, given $\delta > \frac{1}{2} \theta(\xi)$, there exists $N^* \in \N$ such that, for each $N \geq N^*$ and $k \in [N,N+\eta]$,
  \begin{equation}
    \begin{aligned}
      \label{eq:dnub_J}
      J_{\sigma_k(\xi')} \bigl( \rho_k(\xi') \bigr) - J_{\sigma_N(\xi)}(\xi') 
      &\leq -\bar{\alpha} \bar{\beta}^N \frac{1}{2} \theta(\xi) \\
      &\leq -\bar{\alpha} \bar{\beta}^N \theta_{\sigma_N(\xi)}(\xi). \\
    \end{aligned}
  \end{equation}
  and at the same time
  \begin{equation}
    \label{eq:dnub_betabar}
    \bar{\alpha} \bar{\beta}^N 
    \leq ( 1 - \omega ) \alpha \beta^{M_\delta^*} 
    \leq ( 1 - \omega ) \alpha \beta^{\mu_{\sigma_N}(\xi)},
  \end{equation}
  where $M_\delta^*$ is as in Lemma \ref{lemma:discrete_mu_upper_bound}.

  Similarly, given ${\cal A}_\tau(\xi) = \left\{ (j,t) \in {\cal J} \times [0,1] \mid \Psi_\tau(\xi) = \psi_{\tau,j,t}(\xi) \right\}$, let $(j,t) \in {\cal A}_{\sigma_N(\xi')}(\xi')$. Thus, for $N \geq N^*$, $k \in [N,N+\eta]$, and using Lemma \ref{lemma:discrete_state_approx},
  \begin{equation}
    \begin{aligned}
      \label{eq:dnub_psi}
      \Psi_{\sigma_k(\xi')} \bigl( \rho_k(\xi') \bigr) - \Psi_{\sigma_N(\xi)}(\xi') 
      &= \psi_{\sigma_k(\xi'),j,t} \bigl( \rho_k(\xi') \bigr) - \Psi_{\sigma_N(\xi)}(\xi') \\
      &\leq \psi_{\sigma_k(\xi'),j,t} \bigl( \rho_k(\xi') \bigr) - \psi_{\sigma_N(\xi),j,t}(\xi') \\
      &\leq L K \left( \frac{1}{\sqrt{2}} \right)^N \left( \| \xi' \|_{BV} + 2 \right) \\
      &\leq - \bar{\alpha} \bar{\beta}^N \theta_{\sigma_N(\xi)}(\xi).
    \end{aligned}
  \end{equation}

  Therefore, for $N \geq N^*$, if $\Psi_{\sigma_N(\xi)}(\xi) \leq 0$, then by Equations \eqref{eq:dnub_J}, \eqref{eq:dnub_psi}, and the inequalities from the computation of $\mu_\tau(\xi)$,
  \begin{gather}
    J_{\sigma_k(\xi')} \bigl( \rho_k(\xi') \bigr) - J_{\sigma_N(\xi)}(\xi) 
    \leq \bigl( \alpha \beta^{\mu_{\sigma_N}(\xi)} - \bar{\alpha} \bar{\beta}^N \bigr) \theta_{\sigma_N(\xi)}(\xi), \\
    \Psi_{\sigma_k(\xi')} \bigl( \rho_k(\xi') \bigr) 
    \leq \bigl( \alpha \beta^{\mu_{\sigma_N}(\xi)} - \bar{\alpha} \bar{\beta}^N \bigr) \theta_{\sigma_N(\xi)}(\xi) \leq 0,
  \end{gather}
  which together with Equation \eqref{eq:dnub_betabar} implies that the feasible set is not empty. 
  Similarly, if $\Psi_{\sigma_N(\xi)}(\xi) > 0$, by Equation \eqref{eq:dnub_psi},
  \begin{equation}
    \Psi_{\sigma_k(\xi')} \bigl( \rho_k(\xi') \bigr) - \Psi_{\sigma_N(\xi)}(\xi) 
    \leq \bigl( \alpha \beta^{\mu_{\sigma_N}(\xi)} - \bar{\alpha} \bar{\beta}^N \bigr) \theta_{\sigma_N(\xi)}(\xi),
  \end{equation}
  as desired.

  Hence for all $N \geq N^*$ the feasible sets of the optimization problems associated with $\nu_{\sigma_N(\xi)}$ are not empty, and therefore $\nu_{\sigma_N(\xi)}( \xi, N + \eta ) < \infty$.
\end{proof}


\begin{lemma}
  \label{lemma:discrete_N_diverges}
  Let $\{ N_i \}_{i \in \N}$, $\{ \tau_i \}_{i \in \N}$, and $\{ \xi_i \}_{i \in \N}$ be the sequences produced by Algorithm \ref{algo:discrete_algo}.
  Then $N_i \to \infty$ as $i \to \infty$.
\end{lemma}
\begin{proof}
  Suppose that $N_i \leq N^*$ for all $i \in \N$. 
  Then, by definition of Algorithm \ref{algo:discrete_algo}, there exists $i_0 \in \N$ such that $\theta(\xi_i) \leq - \Lambda 2^{-\chi N_i} \leq - \Lambda 2^{-\chi N^*}$ and $\xi_{i+1} = \Gamma_{\tau_i}(\xi_i)$ for each $i \geq i_0$, where $\Gamma_\tau$ is defined in Equation \eqref{eq:discrete_gamma}. 
  
  Moreover, by definition of $\nu_\tau$ we have that if there exists $i_1 \geq i_0$ such that $\Psi_{\tau_{i_1}} ( \xi_{i_1} ) \leq 0$, then $\Psi_{\tau_i}( \xi_i ) \leq 0$ for each $i \geq i_1$.
  Let us assume that there exists $i_1 \geq i_0$ such that $\Psi_{\tau_{i_1}} ( \xi_{i_1} ) \leq 0$, then, using Lemma \ref{lemma:discrete_mu_upper_bound},
  \begin{equation}
    \begin{aligned}
      J_{\tau_{i+1}} ( \xi_{i+1} ) - J_{\tau_i} ( \xi_i ) 
      &\leq \bigl( \alpha \beta^{\mu_{\tau_i}(\xi_i)} - \bar{\alpha} \bar{\beta}^{\nu_{\tau_i}(\xi_i,N_i+\eta)} \bigr) \theta(\xi_i) \\
      &\leq - \omega \alpha \beta^{M^*_{\delta'}} \delta',
    \end{aligned}
  \end{equation}
  for each $i \geq i_1$, where $\delta' = \Lambda 2^{-\chi N^*}$. 
  But this implies that $J_{\tau_i}(\xi_i) \to -\infty$ as $i \to \infty$, which is a contradiction since $h_0$, and therefore $J_{\tau_i}$, is lower bounded.
  
  The argument is completely analogous in the case where the sequence is perpetually infeasible. Indeed, suppose that $\Psi_{\tau_i}( \xi_i ) > 0$ for each $i \geq i_0$, then by Lemma \ref{lemma:discrete_mu_upper_bound},
  \begin{equation}
    \begin{aligned}
      \Psi_{\tau_{i+1}} ( \xi_{i+1} ) - \Psi_{\tau_i} ( \xi_i ) 
      &\leq \bigl( \alpha \beta^{\mu_{\tau_i}(\xi_i)} - \bar{\alpha} \bar{\beta}^{\nu_{\tau_i}(\xi_i,N_i+\eta)} \bigr) \theta(\xi_i) \\
      &\leq - \omega \alpha \beta^{M^*_{\delta'}} \delta',      
    \end{aligned}
  \end{equation}
  for each $i \geq i_0$, where $\delta' = \Lambda 2^{-\chi N^*}$.
  But again this implies that $\Psi_{\tau_i}(\xi_i) \to -\infty$ as $i \to \infty$, which is a contradiction since we had assumed that $\Psi_{\tau_i}( \xi_i ) > 0$.
\end{proof}


\begin{lemma}
  \label{lemma:discrete_phase12}
  Let $\{ N_i \}_{i \in \N}$, $\{ \tau_i \}_{i \in \N}$, and $\{ \xi_i \}_{i \in \N}$ be the sequences produced by Algorithm \ref{algo:discrete_algo}.
  Then there exists $i_0 \in \N$ such that, if $\Psi_{\tau_{i_0}}( \xi_{i_0} ) \leq 0$, then $\Psi( \xi_i ) \leq 0$ and $\Psi_{\tau_i}( \xi_i ) \leq 0$ for each $i \geq i_0$.
\end{lemma}
\begin{proof}
  Let ${\cal I} \subset \N$ be a subsequence defined by
  \begin{equation}
    \label{eq:dp12_Idef}
    {\cal I} = \left\{ i \in \N \mid 
      \theta_{\tau_i}(\xi_i) \leq - \frac{\Lambda}{2^{\chi N_i}}\ \text{and}\ 
      \nu_{\tau_i}(\xi_i,N_i + \eta) < \infty \right\}.    
  \end{equation}
  Note that, by definition of Algorithm \ref{algo:discrete_algo}, $\Psi(\xi_{i+1}) = \Psi(\xi_i)$ for each $i \notin {\cal I}$. 
  Now, for each $i \in {\cal I}$ such that $\Psi_{\tau_i}(\xi_i) \leq 0$, by definition of $\nu_\tau$ in Equation \eqref{eq:discrete_nu} together with Corollary \ref{corollary:discrete_mu_upper_bound},
  \begin{equation}
    \begin{aligned}
      \Psi_{\tau_{i+1}}(\xi_{i+1}) 
      &\leq \left( \alpha \beta^{\mu_{\tau_i}(\xi_i)} - \bar{\alpha} \bar{\beta}^{\nu_{\tau_i}(\xi_i,N_i+\eta)} \right) \theta_{\tau_i}(\xi_i) \\
      &\leq - \omega \alpha \beta^{\mu_{\tau_i}(\xi_i)} \frac{\Lambda}{ 2^{\chi N_i} } \\
      &\leq - \omega \alpha \beta C \left( \frac{\Lambda}{ 2^{\chi N_i} } \right)^2,
    \end{aligned}
  \end{equation}
  where $C > 0$.
  By Lemma \ref{lemma:roc_constraint} and the fact that $N_{i+1} \geq N_i$, we have that
  \begin{equation}
    \label{eq:dp12_psi_bound}
    \begin{aligned}
      \Psi( \xi_{i+1} ) 
      &\leq \frac{B}{2^{N_i}} - \omega \alpha \beta C \left( \frac{\Lambda}{ 2^{\chi N_i} } \right)^2 \\
      &\leq \frac{1}{ 2^{2 \chi N_i} } \left( \frac{B}{ 2^{ ( 1 - 2 \chi ) N_i } } - \omega \alpha \beta C \Lambda^2 \right).
    \end{aligned}
  \end{equation}
  Hence, if $\Psi_{\tau_{i_1}}( \xi_{i_1} ) \leq 0$ for $i_1 \in \N$ such that $N_{i_1}$ is large enough, then $\Psi( \xi_i ) \leq 0$ for each $i \geq i_1$.

  Moreover, from Equation \eqref{eq:dp12_psi_bound} we get that for each $N \geq N_i$ and each $\tau \in {\cal T}_N$,
  \begin{equation}
    \label{eq:dp12_psitau_bound}
    \begin{aligned}
      \Psi_\tau( \xi_{i+1} ) 
      &\leq \frac{1}{ 2^{2 \chi N_i} } \left( \frac{B}{ 2^{ ( 1 - 2 \chi ) N_i } } - \omega \alpha \beta C \Lambda^2 \right) + \frac{B}{2^N} \\
      &\leq \frac{1}{ 2^{2 \chi N_i} } \left( \frac{2B}{ 2^{ ( 1 - 2 \chi ) N_i } } - \omega \alpha \beta C \Lambda^2 \right).
    \end{aligned}
  \end{equation}
  Thus, if $\Psi_{\tau_{i_2}}( \xi_{i_2} ) \leq 0$ for $i_2 \in \N$ such that $N_{i_2}$ is large enough, then $\Psi_\tau( \xi_{i_2} ) \leq 0$ for each $\tau \in {\cal T}_N$ such that $N \geq N_i$. 
  But note that this is exactly the case when $i_2+k \notin {\cal I}$ for $k \in \{1,\ldots,n\}$, thus we can conclude that $\Psi_{\tau_{i_2+k}}( \xi_{i_2+k} ) \leq 0$. 
  Also note that the case of $i \in {\cal I}$ is trivially satisfied by the definition of $\nu_\tau$.

  Finally, by setting $i_0 = \max\{ i_1, i_2 \}$ we get the desired result.
\end{proof}


\begin{theorem}
  \label{thm:discrete_convergence}
  Let $\{ N_i \}_{i \in \N}$, $\{ \tau_i \}_{i \in \N}$, and $\{ \xi_i \}_{i \in \N}$ be the sequences produced by Algorithm \ref{algo:discrete_algo}. 
  Then $\theta_{\tau_i}(\xi_i) \to 0$ as $i \to \infty$.
\end{theorem}
\begin{proof}
  Let us suppose that $\lim_{i \to \infty} \theta_{\tau_i}( \xi_i ) \neq 0$. Then there exists $\delta > 0$ such that
  \begin{equation}
    \liminf_{i \to \infty} \theta_{\tau_i}( \xi_i ) < -4 \delta,
  \end{equation}
  and hence, using Lemmas \ref{lemma:discretized_theta_convergence} and \ref{lemma:discrete_N_diverges}, there exists an infinite subsequence ${\cal K} \subset \N$ defined by
  \begin{equation}
    \label{eq:dconv_Kdef}
    {\cal K} = \bigl\{ i \in \N \mid 
      \theta_{\tau_i}(\xi_i) < -2 \delta \ \text{and}\ \theta(\xi_i) < - \delta \bigr\}.
  \end{equation}

  Let us define a second subsequence ${\cal I} \subset \N$ by
  \begin{equation}
    \label{eq:dconv_Idef}
    {\cal I} = \left\{ i \in \N \mid 
      \theta_{\tau_i}(\xi_i) \leq - \frac{\Lambda}{2^{\chi N_i}}\ \text{and}\ 
      \nu_{\tau_i}(\xi_i,N_i + \eta) < \infty \right\}.
  \end{equation}
  Note that by the construction of the subsequence ${\cal K}$, together with Lemma \ref{lemma:discrete_nu_upper_bound}, we get that ${\cal K} \cap {\cal I}$ is an infinite set.

  Now we will analize Algorithm \ref{algo:discrete_algo} by considering the behavior of each step as a function of its membership to each subsequence.
  First, for each $i \notin {\cal I}$, $\xi_{i+1} = \xi_i$, thus $J( \xi_{i+1} ) = J( \xi_i )$ and $\Psi( \xi_{i+1} ) = \Psi( \xi_i )$.
  Second, let $i \in {\cal I}$ such that $\Psi_{\tau_i}(\xi_i) \leq 0$, then
  \begin{equation}
    \begin{aligned}
      J_{\tau_{i+1}}(\xi_{i+1}) - J_{\tau_i}(\xi_i) 
      &\leq \left( \alpha \beta^{ \mu_{\tau_i}(\xi_i) } - \bar{\alpha} \bar{\beta}^{ \nu_{\tau_i}(\xi_i,N_i+\eta) } \right) 
            \theta_{\tau_i}( \xi_i ) \\
      &\leq - \omega \alpha \beta^{ \mu_{\tau_i}(\xi_i) } \frac{\Lambda}{2^{\chi N_i}} \\
      &\leq - \omega \alpha \beta C \left( \frac{\Lambda}{2^{\chi N_i}} \right)^2,
    \end{aligned}
  \end{equation}
  where $C > 0$ and the last inequality follows from Corollary \ref{corollary:discrete_mu_upper_bound}. 
  Recall that $N_{i+1} \geq N_i$, thus using Lemmas \ref{lemma:roc_cost} and \ref{lemma:discrete_N_diverges} we have that 
  \begin{equation}
    \begin{aligned}
      J(\xi_{i+1}) - J(\xi_i)
      &\leq \frac{2B}{2^{N_i}} - \omega \alpha \beta C \left( \frac{\Lambda}{2^{\chi N_i}} \right)^2 \\
      &\leq \frac{1}{ 2^{2 \chi N_i} } \left( \frac{2B}{ 2^{ (1 - 2 \chi) N_i } } - \omega \alpha \beta C \Lambda^2 \right),
    \end{aligned}
  \end{equation}
  and since $\chi \in \left( 0, \frac{1}{2} \right)$, we get that for $N_i$ large enough $J(\xi_{i+1}) \leq J(\xi_i)$.
  % Also, using the same argument and Lemma \ref{lemma:roc_constraint},
  % \begin{equation}
  %   \Psi( \xi_{i+1} ) 
  %   \leq \frac{1}{ 2^{2 \chi N_i} } \left( \frac{2B}{ 2^{ (1 - 2 \chi) N_i } } - \omega \alpha \beta C \Lambda^2 \right),
  % \end{equation}
  % which implies that, for $N_i$ large enough, $\Psi(\xi_{i+1}) \leq 0$.
  Similarly, if $\Psi_{\tau_i}(\xi_i) > 0$ then
  \begin{equation}
    \Psi(\xi_{i+1}) - \Psi(\xi_i)
    \leq \frac{1}{ 2^{2 \chi N_i} } \left( \frac{2B}{ 2^{ (1 - 2 \chi) N_i } } - \omega \alpha \beta C \Lambda^2 \right),    
  \end{equation}
  thus for $N_i$ large enough, $\Psi(\xi_{i+1}) \leq \Psi(\xi_i)$.
  Third, let $i \in {\cal K} \cap {\cal I}$ such that $\Psi_{\tau_i}(\xi_i) \leq 0$, then, by Lemma \ref{lemma:discrete_mu_upper_bound},
  \begin{equation}
    \begin{aligned}
      J_{\tau_{i+1}}(\xi_{i+1}) - J_{\tau_i}(\xi_i) 
      &\leq \left( \alpha \beta^{ \mu_{\tau_i}(\xi_i) } - \bar{\alpha} \bar{\beta}^{ \nu_{\tau_i}(\xi_i,N_i+\eta) } \right) 
            \theta_{\tau_i}( \xi_i ) \\
      &\leq - 2 \omega \alpha \beta^{ M^*_{2 \delta} } \delta,
    \end{aligned}
  \end{equation}
  thus, by Lemmas \ref{lemma:roc_cost} and \ref{lemma:discrete_N_diverges}, for $N_i$ large enough,
  \begin{equation}
    \label{eq:dconv_J_KI}
    J(\xi_{i+1}) - J(\xi_i) 
    \leq - \omega \alpha \beta^{ M^*_{2 \delta} } \delta.
  \end{equation}
  Similarly, if $\Psi_{\tau_i}(\xi_i) > 0$, using the same argument and Lemma \ref{lemma:roc_constraint}, for $N_i$ large enough,
  \begin{equation}
    \label{eq:dconv_Psi_KI}
    \Psi(\xi_{i+1}) - \Psi(\xi_i) 
    \leq - \omega \alpha \beta^{ M^*_{2 \delta} } \delta.
  \end{equation}

  Now let us assume that there exists $i_0 \in \N$ such that $N_{i_0}$ is large enough and $\Psi_{\tau_{i_0}}(\xi_{i_0}) \leq 0$. 
  Then by Lemma \ref{lemma:discrete_phase12} we get that $\Psi_{\tau_i}( \xi_i ) \leq 0$ for each $i \geq i_0$.
  But as shown above, either $i \notin {\cal K} \cap {\cal I}$ and $J(\xi_{i+1}) \leq J(\xi_i)$ or $i \in {\cal K} \cap {\cal I}$ and Equation \eqref{eq:dconv_J_KI} is satisfied, and since ${\cal K} \cap {\cal I}$ is an infinite set we get that $J(\xi_i) \to - \infty$ as $i \to \infty$, which is a contradiction as $J$ is lower bounded.

  On the other hand, if we assume that $\Psi_{\tau_i}(\xi_i) > 0$ for each $i \in \N$, then either $i \notin {\cal K} \cap {\cal I}$ and $\Psi(\xi_{i+1}) \leq \Psi(\xi_i)$ or $i \in {\cal K} \cap {\cal I}$ and Equation \eqref{eq:dconv_Psi_KI} is satisfied, thus implying that $\Psi(\xi_i) \to -\infty$ as $i \to \infty$.
  But this is a contradiction since, by Lemma \ref{lemma:roc_constraint}, this would imply that $\Psi_{\tau_i}(\xi_i) \to - \infty$ as $i \to \infty$.

  Finally, both contradictions imply that $\theta_{\tau_i}(\xi_i) \to 0$ as $i \to \infty$ as desired.
\end{proof}


==> Sections/epiconvergence.tex <==
\subsection{Epiconvergence}

Let $\overline{\R} = \R \cup \{-\infty,\infty\}$. We begin by defining the epigraph of the original problem:
\begin{equation}
	\label{eq:epigraph}
	E = \{ \left(x,\xi\right) \subset \overline{\R} \times {\cal X}_p \;|\; x \geq J(\xi),\; \psi(\xi) \leq 0\}.
\end{equation}
For a positive integer $N$ and a switching vector $\tau \in {\cal T}_N$, we define the epigraph of the discretized problem similarly:
\begin{equation}
	\label{eq:discretized_epigraph}
	E_{\tau} = \{ \left(x,\xi\right) \subset \overline{\R} \times {\cal X}_{p,\tau} \;|\; x \geq J_{\tau}(\xi),\; \psi_{\tau}(\xi) \leq 0\}.
\end{equation}

\begin{definition}
	\label{def:epiconvergence}
	Let $\{\tau_i\}_{i\in \N}$ be a sequence where $\tau_i \in {\cal T}_i$ and $\{E_i\}_{i\in \N}$ be a sequence of epigraphs associated with each of the switching vectors. We say that a sequence $\{E_i\}_{i\in\N}$ \emph{epiconverges} to $E$ if:
	\begin{enumerate_parentesis}
		\item \label{def:epi_limsup} for every $\xi \in {\cal X}_p$ such that $\psi(\xi) \leq 0$, there exists a sequence $\{\xi_i\}_{i\in \N}$ with $\xi_i \in {\cal X}_{p,\tau_i}$ and $\psi_{\tau_i}(\xi_i) \leq 0$ for each $i$ in $\N$, such that $\lim_{i\to\infty}\xi_i=\xi$ and $\limsup_{i \to \infty} J_{\tau_i}(\xi_i) \leq J(\xi)$, and
		\item \label{def:epi_liminf} for every infinite sequence $\{\xi_i\}_{i\in\N}$ with $\lim_{i\to\infty}\xi_i=\xi$, $\xi_i \in {\cal X}_{p,\tau_i}$ and $\psi_{\tau_i}(\xi_i) \leq 0$ for each $i$ in $\N$, then $\xi \in {\cal X}_p$, $\psi(\xi) \leq 0$, and $\liminf_{i\to\infty} J_{\tau_i}(\xi_i) \geq J(\xi)$.
	\end{enumerate_parentesis}
\end{definition}

\begin{theorem}[Polak \cite{Polak1997} Theorem 3.3.3]
	\label{thm:epiconvergence}
	Let $\{\tau_i\}_{i\in \N}$ be a sequence where $\tau_i \in {\cal T}_i$ and $\{E_i\}_{i\in \N}$ be a sequence of epigraphs associated with each of the switching vectors. Suppose $\{E_i\}_{i\in\N}$ epiconverges to $E$, then:
	\begin{enumerate_parentesis}
		\item \label{thm:global_minimizers} If $\{\xi_i\}_{i\in\N}$ is a sequence of global minimizers for each of the discretized hybrid optimal control problems induced by switching vector $\tau_i$, and $\xi$ is any accumulation point of this sequence then, $\xi$ is a global minimizer of the original hybrid optimal control problem. 
		\item \label{thm:local_minimizers} If $\{\xi_i\}_{i\in\N}$ is a sequence of local minimizers for each of the discretized hybrid optimal control problems induced by switching vector $\tau_i$, sharing a common radius of attraction and $\xi$ is any accumulation point of this sequence then, $\xi$ is a local minimizer of the original hybrid optimal control problem.
	\end{enumerate_parentesis}
\end{theorem}

\begin{assumption}
	\label{assump:constraint_qualification}
	Let $\psi: {\cal X}_p \to \R$ be defined as in Equation \eqref{eq:super_const}, then for every $\xi \in {\cal X}_p$ such that $\psi(\xi) \leq 0$, there exists a sequence, $\{\xi_i\}_{i\in \N} \subset {\cal X}_p$, such that $\psi(\xi_i) < 0$ for all $i$ in $\N$ and $\lim_{i\to\infty} \xi_i = \xi$.
\end{assumption}

\begin{theorem}
	\label{thm:ourproblem_epiconverges}
	Let $\{\tau_i\}_{i\in \N}$ be a sequence where $\tau_i \in {\cal T}_i$ and $\{E_i\}_{i\in \N}$ be a sequence of epigraphs associated with each of the switching vectors, then $\{E_i\}_{i\in\N}$ epiconverges to $E$.
\end{theorem}
\begin{proof}
	We begin by first proving Condition \ref{def:epi_limsup} in Definition \ref{def:epiconvergence}. Let $\xi \in {\cal X}_p$ be arbitrary. By Assumption \ref{assump:constraint_qualification}, there exists a sequence $\{\xi_i\}_{i\in\N} \subset {\cal X}_p$ such that $\lim_{i\to\infty}\xi_i=\xi$ and $\psi(\xi_i) < 0$ for all $i \in \N$. From Lemma \ref{lemma:roc_constraint} that there exists a $K > 0$ such that for all $\xi' \in {\cal X}_{p,\tau_i}$:
	\begin{equation}
		\label{eq:epiconverges_a}
		\left|\psi_{\tau_i}(\xi') - \psi(\xi') \right| \leq \frac{K}{2^i}.
	\end{equation}
	Clearly, for each $i$ there exists a $j_i \in \N$ and a $\xi'_{j_i} \in {\cal X}_{p,\tau_{j_i}}$ such that: (a) $\frac{K}{2^{j_i}} \leq -\frac{\psi(\xi_i)}{2}$, (b) $\left\| \xi'_{j_i} - \xi_i \right\|_{\cal X} \leq \frac{1}{2^i}$, (c) $\psi(\xi'_{j_i}) \leq \frac{\psi(\xi_i)}{2}$, and (d) $j_i < j_{i+1}$ for all $i \in \N$. Obviously, $\xi'_{j_i} \in {\cal X}_{p,\tau_{j_i+k}}$ for all $k \in \N$. It follows from Equation \eqref{eq:epiconverges_a} that $\psi_{\tau_{j_i+k}}(\xi'_{j_i}) \leq 0$ for any $i,k \in \N$. Now consider the sequence $\{\xi^*_l\}_{l=j_1}^{\infty}$, defined as follows: $\xi^*_l = \xi'_{j_i}$ for $l = j_i,j_i+1,\ldots,j_{i+1}-1$, $i = 1,2,\ldots$. Clearly $\psi_{\tau_l}(\xi^*_l)\leq 0$, for all $l \geq j_1$, and $\lim_{l\to\infty}\xi_l=\xi$.  Employing Lemma \ref{lemma:roc_cost} and the continuity of $J$ as is proven in Corollary \ref{corollary:J_continuous}, we conclude that $\lim_{l\to\infty}J_{\tau_l}(\xi^*_l) = J(\xi)$, which proves Condition \ref{def:epi_limsup} in Definition \ref{def:epiconvergence}.
	
	Next, suppose that $\{\xi_i\}_{i\in\N}$, with $\xi_i \in {\cal X}_{p,\tau_i}$ is such that $\psi_{\tau_i}(\xi_i) \leq 0$ for all $i \in \N$ and $\lim_{i\to\infty}\xi_i=\xi$. By Lemma \ref{lemma:dense_pure_discretized_space}, $\xi \in {\cal X}_{p}$. Next, by the continuity of $\psi$, as is shown in Lemma \ref{lemma:psi_continuous}, and Lemma \ref{lemma:roc_constraint} $\psi(\xi) \leq 0$. Moreover, by the continuity of $J$, as is shown in Corollary \ref{corollary:J_continuous}, and Lemma \ref{lemma:roc_cost}, $\lim_{i\to\infty}J(\xi_i) = J(\xi)$, which shows that Condition \ref{def:epi_liminf} in Definition \ref{def:epiconvergence} is satisfied. Therefore we have our desired result.
	
\end{proof}




==> Sections/implementation.tex <==
\section{Algorithm Implementation}
\label{sec:implementation}

In this section, we describe how to implement Algorithm \ref{algo:main_algo} given the various algorithmic components derived in the Section \ref{sec:algo_analysis}. 
Numerically computing a solution to the Switched System Optimal Control Problem defined as in Equation \eqref{eq:ssocp} demands employing some form of discretization. 
When numerical integration is introduced, the original infinite-dimensional optimization problem defined over function spaces is replaced by a finite-dimensional discrete-time optimal control problem. 
Changing the discretization precision results in an infinite sequence of such approximating problems. 
Our goal is the construction of an implementable algorithm that generates a sequence of points by recursive application that converge to a point that satisfies the optimality condition defined in Equation \eqref{eq:theta_definition}.

In this section, we begin by describing our discretization strategy, which allows us to define our discretized optimization spaces. Next, we describe how to construct discretized trajectories, cost, constraints, and optimal control problems. We conclude by constructing our numerically implementable optimal control algorithm for switched systems.

\input{Sections/discretization.tex}
% \input{Sections/epiconvergence.tex}
\input{Sections/consistent_approximation.tex}
